Computing Maximum Fixed Point Solutions over Feasible Paths in Data Flow Analyses

The control flow graph (CFG) representation of a procedure used by virtually all flow-sensitive program analyses, admits a large number of infeasible control flow paths i.e., these paths do not occur in any execution of the program. Hence the information reaching along infeasible paths in an analysis is spurious. This affects the precision of the conventional maximum fixed point (MFP) solution of the data flow analysis, because it includes the information reaching along all control flow paths. The existing approaches for removing this imprecision are either specific to a data flow problem with no straightforward generalization or involve control flow graph restructuring which may exponentially blow up the size of the CFG. We lift the notion of MFP solution to define the notion of feasible path MFP (FPMFP) solutions that exclude the data flowing along known infeasible paths. The notion of FPMFP is generic and does not involve CFG restructuring. Instead, it takes externally supplied information about infeasible paths and lifts any data flow analysis to an analysis that maintains the distinctions between different paths where these distinctions are beneficial, and ignores them where they are not. Thus it gets the benefit of a path-sensitive analysis where it is useful without performing a conventional path-sensitive analysis. We evaluated the proposed feasible path MFP solutions for reaching definitions analysis and potentially uninitialized variable analysis on 30 benchmarks. The evaluation results indicate that precision improvement in these two analyses respectively reduce the number def-use pairs by up to 13.6% (average 2.87%, geometric mean 1.75%), and reduce the potentially uninitialized variable alarms by up to 100% (average 18.5%, geo. mean 3%). We found that the FPMFP computation time was 2.9X of MFP computation time on average.

==> conclusion.tex <==
\section{Conclusions and Future Work}\label{sec:Conclusion}
An exhaustive data flow analysis answers all queries of a particular type over all possible executions of a program. However, in 
practice it is hard to see an exhaustive analysis that is efficient and computes a precise result, because of the following 
issues that often have conflicting solutions.
\begin{itemize}
\item Issue 1: to achieve efficiency, the analysis may need to merge the information reaching at a program point along different paths, 
because the number of paths as well as the corresponding data flow information may be very large or even unbounded.
\item Issue 2: to achieve precision, the analysis may need to distinguish between the information reaching from different paths, in order to 
1) discard the information reaching along infeasible paths, and 2) avoid potential loss of information because of merging that 
happens at join points of two or more paths.
\end{itemize}

These issues have been handled in past as follows: the first issue is handled by using a \cfg representation for exhaustive data 
flow analysis where the information at the shared segments of different paths is merged. However, it may loose out 
on precision, if the information from different paths is indiscriminately merged. 

To handle the second issue, two types of approaches have been proposed. 
\begin{enumerate}
\item The first approach restructures the \cfg of a procedure so that
the resultant \cfg does not contain infeasible paths, or join points that cause imprecision. However this approach may
blow up the size of the \cfg. 
\item The second approach, selectively annotates data flow values with the path conditions 
that represent the path followed by the data flow values. Next, if a path condition is found to be unsatisfiable then the corresponding
data flow values are discarded. Heuristics are used to decide which path conditions are to be tracked. However, these heuristics are 
mostly analysis specific and may lead to repeated effort for identification of infeasible paths for different data flow analyses performed
on the same underlying program.
\end{enumerate}

In this work, we proposed to remove the effect of infeasible paths from \mfp solutions (a widely used solution of an exhaustive data 
flow analysis), while maintaining the efficiency and generic nature 
of the \mfp computation. We proposed the notion of feasible path \mfp solutions that exclude the data flow values reaching along infeasible 
paths. A key insight
that enabled \fpmfp is that infeasible paths is a property of programs and not of any particular data flow analysis over the programs. 
Hence, we can separate the identification of infeasible paths in the \cfg of a program, from discarding the corresponding data flow values 
during a data flow analysis. This separation allowed us to devise a generic technique for
removing the effect of infeasible paths.

Our empirical evidence suggests that the \fpmfp computation cost was $\avgTime\times$ of the \mfp computation cost.
In our experience, this cost is acceptable considering the potential improvement in the 
precision of an analysis leading to reduced manual effort, for example, in program testing for ensuring the coverage of def-use pairs, 
and validating uninitialized variable alarms.


A possible direction of future work can be to relax (or remove) the restrictions on the inter-procedural \mips that we admit in 
\fpmfp computation. Additionally, it would be interesting to explore the possibility of a lightweight pre-analysis to 
anticipate the cost and precision tradeoff of \fpmfp over \mfp for a input program. Lastly, more program properties (like infeasible paths)
 that are independent of a data flow analysis can be identified and used to improve data flow precision in a generic manner.

%Existing approaches of 
%exhaustive data flow analysis that attempt to remove the effect of infeasible paths resort to one of the following ways.
%\begin{enumerate}
%\item They restructure the \cfg so that the resultant \cfg does not contain infeasible \cfps, or
%\item They annotate data flow values with path conditions that represent the path followed by the data flow values in 
%a data flow analysis. If the path condition is found to be unsatisfiable the corresponding data flow value is not 
%propagated down the path.
%\end{enumerate}

%The former approach of \cfg restructuring is generic i.e., any data flow analysis that uses the restructured \cfg does not include 
%the data flow values along known infeasible \cfps. However, \cfg restructuring is itself costly and can blow up the size of \cfg 
%exponentially. The latter approach that involves path condition needs heuristics to restrict the path conditions that are tracked, 
%otherwise it may end up tracking all path conditions which may or may not lead to infeasible paths. It uses 
%constraint solving to check the satisfiability of the path conditions. Moreover, this approach may repeatedly check the satisfiability 
%of the same path conditions for different data flow analyses performed on the same underlying analysis.
 
%In this work, we proposed the notion of feasible path \mfp that combines the best of the above two approaches i.e., it is generic and
%does not involve \cfg restructuring. A key enabler of the \fpmfp solution is our observation that infeasible paths is a property of
%programs and not of any data flow analysis over programs. Hence, we can separate the identification of infeasible paths from eliminating
%the data flow values that reach along infeasible \cfps. This allows us to reduce the cost of our analysis compared to path annotation based
%approaches. Our analysis uses optimizations to discard the distinctions based on data flow values computed by a data flow analysis
%while still being generic this reduces the analysis cost which is not possible in \cfg restructuring 
%based approaches.

\begin{comment}
Achieving a balance between scalability and precision in data flow analysis is a difficult art. In this work, we proposed the notion of
 feasible path \mfp that achieves a unique tradeoff of scalability and precision, is as generically applicable as \mfp solutions, 
offers better precision than \mfp solutions, and its computation is decidable unlike \mop and \mofp. In some cases, it can also be more precise 
than the \mop solution.

In \fpmfp, we identify the number of distinctions that need to be made between data flow values reaching a 
program along different \cfps. Towards this end, we use the concept of minimal infeasible path segments that tell
us which information is blocked by an infeasible \cfp and where. This allows us to lift any data flow analysis to a
data flow analysis over $k+1$ \pairnames (or $k+1$ parallel, but interacting data flow analyses), where $k$ is the 
total number of \mips in the \cfg. 

A careful design of edge flow function that shifts the values from one \pairname to other \pairname 
at the start and end of a \mips allows us to maintain the distinctions where they are beneficial.
Our experiments on reaching definition analysis and uninitialized variable analysis show a precision gain of up to \uptoDefUse, and 
\uptoUninit\ respectively, with up to 3$\times$ performance degradation in terms of the analysis time. Thus,
\fpmfp solution is a sweet spot between two extremes: efficient but imprecise \mfp solution on the one hand and
extremely inefficient but very precise \mofp solution. 

In our experience, the additional cost incurred in a \fpmfp computation is acceptable considering the potential improvement in the 
precision of the analyses leading to reduced manual effort, for example, in program testing for ensuring the coverage of def-use pairs, 
and validating uninitialized variable alarms.

\KPadd{An immediate future work is to relax (or remove) the restrictions on the inter-procedural \mips that we admit in  \fpmfp computation. 
Additionally, it would be interesting to explore the possibility of a lightweight pre-analysis to 
anticipate the cost and precision tradeoff of \fpmfp over \mfp for a input program. Lastly, infeasible path is a property of a 
program instead of a data flow analysis; this distinction allowed us to design an analysis independent technique to remove the effect of 
infeasible \cfps, in future, more such program properties can be identified and used to improve data flow precision. }
\end{comment}

==> relatedWork.tex <==
\section{Related Work}\label{sec:Relatedwork}

Presence of the infeasible paths in the programs is well known~
\cite{zhu2019detecting,hedley1985causes,malevris1990predictive,lee2019infeasible,jiang2019approach,gong2019detecting,sewell2016complete,
zeng2017type}. 
Hedley et al. presented a detailed analysis of the causes and 
effects of the infeasible paths in programs~\cite{hedley1985causes}. Malevris et al. observed that the greater the number of conditional 
statements contained in a path, the greater the probability of the path being infeasible~\cite{malevris1990predictive}. 
Bodik et al. found that around 9-40\% of the conditional statements in programs show statically detectable correlation 
with infeasible control flow paths~\cite{bodik1997refining} 

Many approaches detect infeasible program paths~\cite{bodik1997refining,bodik1997interprocedural,ngo2007detecting,rui2006infeasible,
delahaye2010explanation,bueno2000identification,zhuang2006using,yang2011improve,bertolino1994automatic,chen2007exploiting,
malevris1990predictive,navabi2010path,yang2020infeasible}.
 For most of these approaches, the goal is to
detect infeasible control flow paths by analyzing the correlations of different conditional statements or between a conditional and an 
assignment statement.

In our work, we used the algorithms proposed by Bodik et al. for detecting infeasible paths~\cite{bodik1997refining} with some
modifications. Our work differs from their work in the way we use the information after infeasible paths are detected. They have applied 
their work for improving the precision of the demand driven def-use analysis. While we proposed a \emph{generic} approach for improving the 
precision of any exhaustive data flow analysis, using the knowledge of the infeasible paths in the program. 
%A desire for such generic approach has been stated in Bodik's work.

Existing approaches that attempt to remove the effect of infeasible paths in data flow analysis are either analysis specific or 
involve \cfg restructuring which can exponentially blow up the size of the \cfg.  The \fpmfp combines the best of both these categories
 because \fpmfp does not involve \cfg restructuring and is generically applicable to all data flow analyses.  We now explain approaches
in either category below.

\subsection{Analysis Specific Approaches}
In literature, analyses like \fpmfp analysis that distinguish between the data flow values reaching along different classes of \cfps, resemble 
to a category 
of analyses called the path sensitive analyses~\cite{das2002esp,dhurjati2006path,hampapuram2005symbolic,xie2003archer,dillig2008sound,
dor2004software}. 

A completely
path sensitive analysis has been tried where each path information is separately tracked along with the corresponding path constraints. 
If the path constraint is found unsatisfiable, the path information is not propagated further. This approach does not scale to most practical 
programs due to presence of loops and recursion leading to an unbounded number of program paths combined with possibly infinite 
data flow lattices.

Selective path sensitive analyses exist in literature~\cite{dor2004software,dillig2008sound,xie2003archer,hampapuram2005symbolic,
dhurjati2006path,das2002esp,thakur2008comprehensive,chen2007exploiting}. They use selective path constraints governed by various 
heuristics for deciding which path information should be kept separately and which path information can be approximated at join 
points. At join points, the data flow information with the same path constraints is merged.

Das et.al, proposed a property specific path sensitive analysis~\cite{das2002esp} in which the information separation 
is maintained only for those paths along which property related behavior changes. 
Dhurjati et.al proposed an iterative path sensitive analysis~\cite{dhurjati2006path} in which the precision is improved 
by finding and adding more effective predicates to the data flow analysis in successive iterations. 
Hampapuram et.al performed a symbolic path simulation approach~\cite{hampapuram2005symbolic} in which they executed 
each path symbolically and propagated the information along these paths. If a path is found infeasible in simulation its 
information is not propagated. A lightweight decision procedure is used to check the feasibility of a path during path simulation.

Xie et.al proposed an approach to detect memory access errors~\cite{xie2003archer}. They use precise path sensitive analysis 
only for constraints and variables which directly or indirectly affect some memory accesses. Dillig et.al introduced the concept 
of observable and unobservable variables to improve the scalability of path sensitive analysis~\cite{dillig2008sound}. 
Dor et.al proposed a precise path sensitive value analysis approach using value bit vectors~\cite{dor2004software}.

Infeasible control flow paths is a property of programs instead of any particular data flow analysis. 
We use this observation to first detect infeasible paths in programs and propose an approach to improve the precision of any data 
flow analysis over the programs, unlike above approaches which remove the impact of infeasible paths from a particular data flow analysis.


Chen et al. proposed an algorithm for detecting infeasible paths incorporating the branch correlations analysis~\cite{rui2006infeasible} 
into the data flow analysis technique, which also improve the precision of traditional data flow analysis. However, their technique cannot 
be generically applied to all data flow analyses.

The trace partitioning approaches~\cite{handjieva1998refining,holley1981qualified,mauborgne2005trace} partition program traces where values 
of some variable or conditional expression differ in two selected traces. The variables or expressions are selected based on the alarms 
to be analyzed or some heuristic. It is similar to our 
approach because it keeps data flow values separately for each partition. However, our approach 
does not rely on alarms, does not need the designer of an analysis to decide a suitable heuristic, 
 and is not restricted to a particular analysis.
We lift partitioning from within an analysis to the infeasibility of control flow paths which is a fundamental
property of control flow paths independent of an analysis. This allow us to
devise an automatic approach to implement a practical trace partitioning.
An interesting aspect of our approach is that although it is oblivious to any analysis, it can be seen as dynamic
partitioning that uses abstract values being computed by an analysis.

\subsection{Approaches that involve \cfg restructuring}

Bodik et al. proposed an interprocedural version of infeasible path detection~\cite{bodik1997interprocedural} and its 
application to improve the data flow precision. However, they use control flow graph restructuring which is not done in our approach. 
\cfg restructuring may blow up the size of the \cfg. Moreover, it does not take the advantage of analysis specific information, 
unlike \fpmfp that uses analysis specific information to dynamically discard the distinctions between \mips, where they do not lead to 
precision improvement as described in Optimization 2 (Section~\ref{sec:optimization.cso}).

Aditya et al. proposed an approach to improve data flow precision by eliminating the destructive merges from control flow graph 
through control flow graph restructuring~\cite{thakur2008comprehensive}. Ammon et.al proposed a similar \cfg restructuring  
 for avoiding information merging along hot paths~\cite{ammons1998improving,ammons2004improving}. However, they did not address 
the imprecision added by infeasible control flow paths.

Mueller et al. used code replication to eliminate conditional branches for achieving faster 
code execution at the cost of increased code size~\cite{mueller1995avoiding}. This approach achieves a similar effect as that of CFG 
restructuring and can blow up the code size exponentially. Hence,  Mueller et al. applied various heuristics to choose the conditionals whose 
elimination lead to faster code execution with less code replication.



==> table1.tex <==
%def-use add for avg computation
%0,0,7.39,8.72,3.50,0.91,1.89,3.24,3.10,0.48,4.67,3.43,12.83,0.49,
%1.40,3.20,2.72,2.78,0.34,5.57,0.91,0.82,2.05,3.52,0.04,1.54,5.21,1.46,3.94,15
%one added to computed geo mean
%1,1,8.39,9.72,4.50,1.91,2.89,4.24,4.10,1.48,5.67,4.43,13.83,1.49,
%2.40,4.20,3.72,3.78,1.34,6.57,1.91,1.82,3.05,4.52,1.04,2.54,6.21,2.46,4.94,16

%overlaps (average 77%)
%0,0,24,85,95,94,93,85,90,92,89,91,88,86,79,94,88,86,88,92,91,90,
%64,68,78,88,63,86,69,89
\begin{table}[ht]%[t]
%\small
%\allowdisplaybreaks
\caption{Reduction in the number of def-use pairs: {\small 1) \mfp (resp. \fpmfp) column shows the sum of number of def-use pairs 
 at all program nodes $n$ in the \cfg of a program for global and local variables. 
%(unlike [2] which only includes local variable def-use pairs). 
2) Three types of benchmarks we used are
  Open source, Industry, and SPEC CPU 2006.
%Benchmarks are 1 to 7 are spec benchmarks, from 8, 9, 10 marked by * are industry code bases
}
}
\label{tab:precision1}
%\setlength{\tabcolsep}{1.8pt}
%\renewcommand{\arraystretch}{1.5}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|l|r|r|r|r|r|r|r|}
\hline
\multicolumn{6}{|c|}{\multirow{1}{*}{Benchmark Properties}} & \multicolumn{3}{c|}{Reaching Definition Analysis}  \\ 
\hline 
\multicolumn{1}{|c|}{\multirow{4}{*}{Type}} &
\multicolumn{1}{|c|}{\multirow{4}{*}{Name}} & \multirow{3}{*}{\parbox{5pt}{\rotatebox{90}{KLOC}}} & \multirow{3}{*}{\parbox{15pt}
{\rotatebox{90}{\#\mipss}}} &\multirow{3}{*}{\parbox{15pt}{\rotatebox{90}{\#Overlapp-}\rotatebox{90}{ing \mipss}}} &\multirow{3}{*}
{\parbox{15pt}{\rotatebox{90}{\%Funcs}\rotatebox{90}{Impacted}}}& \multicolumn{2}{c|}{\#def-use pairs} & 
\multicolumn{1}{c|}{reduction(\%)} 
\\  \cline{7-8}
\multicolumn{1}{|c|}{}&
\multicolumn{1}{|c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}& 
\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}\\%\cline{7-8}
 &&& & & &  \mfp & \multicolumn{1}{c|}{\fpmfp} & \multicolumn{1}{c|}{} \\ 
\hline
%-----------------------------------------------------------------------------------------------------------------------------
\multicolumn{1}{|c|}{\multirow{10}{*}{\rotatebox{90}{Open Source}}}
&1.acpid & 0.3 		     & 17 & 17&15  & 156 & 156 & 0(0.00)\\ \cline{2-9}
&2.polymorph 0.96&0.43  & 24 & 24&17  & 228 & 228 & 0(0.00)\\ \cline{2-9}
&3.nlkain & 0.5 				 & 33 & 8&58   & 1042 & 965 & 77(7.39)\\ \cline{2-9}
&4.spell & 0.6 				 & 21 & 18&23  & 516 & 471 & 45(8.72)\\ \cline{2-9}
&5.ncompress & 1  		   & 47 & 45&30  & 1201 & 1159 & 42(3.50)\\ \cline{2-9}
&6.gzip &1.3 				   & 91 & 86&41 & 3423 & 3392 & 31(0.91)\\ \cline{2-9}
&7.stripcc & 2.1  	     & 142 &133  &35   & 2703 & 2652 & 51(1.89)\\ \cline{2-9}
&8.barcode-nc & 2.3   & 84 & 72&33  & 3051 & 2952 & 99(3.24)\\ \cline{2-9}
&9.barcode & 2.8        & 112 & 101&32   & 3709 & 3594 & 115(3.10)\\ \cline{2-9}
&10.archimedes & 5  		 & 457 & 422&61  & 44337 & 44124 & 213(0.48)\\ \cline{2-9}
&11.combine & 5.7 		   & 301 & 270&39   & 16618 & 15842 & 776(4.67)\\ \cline{2-9}
&12.httpd & 5.7 		     & 252 & 231&17   & 10475 & 10116 & 359(3.43)\\ \cline{2-9}%TFT
&13.sphinxbase & 6.6  	 & 216 & 192&20   & 9641 & 8404 & 1237(12.83)\\ \cline{2-9}
&14.chess & 7.5  		     & 567 & 492&45  & 31386 & 31231 & 155(0.49)\\ \cline{2-9}
&15.antiword &19.3       & 525 & 417&33  & 68889 & 67926 & 963(1.40)\\ \cline{2-9}%TFF
&16.sendmail & 20.3      & 958 & 908&38  & 102812 & 99517 & 3295(3.20)\\ \cline{2-9}%TFT
&17.sudo &45.8           & 402 &355  &29  & 14391 & 13999 & 392(2.72)\\ \cline{2-9}
&18.ffmpeg & 80  	       & 1246 & 1075&10  & 89148 & 86671 & 2477(2.78)\\ \hline%TT2f
\multicolumn{1}{|c|}{\multirow{7}{*}{SPEC}}
&19.mcf & 5.4  		&26&23	&29        & 3570 & 3558 & 12(0.34)       \\ \cline{2-9}
&20.bzip2 & 16 		&712&660		&43    & 82548 & 77947 & 4601(5.57)       \\ \cline{2-9}
&21.hmmer & 16.5   & 888 & 812&25    & 70597 & 69957 & 640(0.91)       \\ \cline{2-9}
&22.sjeng & 27 		&1504&1359	&40    & 77602 & 76966 & 636(0.82)       \\ \cline{2-9}%tt2f
&23.milc & 30  		&685&445		&42    & 18133 & 17762 & 371(2.05)        \\ \cline{2-9}
&24.h264ref & 35.9 & 1920 & 1314&32  & 426346 & 411332 & 15014(3.52)        \\ \cline{2-9}%tt2f
&25.gobmk & 150    & 1921 & 1508&13   & 213243 & 184142 & 29101(13.65)\\ \hline%tt2f
\multicolumn{1}{|c|}{\multirow{3}{*}{Industry}}
&26.NZM &2.7    & 86 & 76&53      & 2652 & 2651 & 1(0.04)  \\ \cline{2-9}
&27.IC &3.7      & 60 & 38&19     & 3111 & 3063 & 48(1.54)  \\ \cline{2-9}
&28.AIS &6 				& 146 & 126&19  & 2475 & 2346 & 129(5.21)  \\ \cline{2-9}%FS 
&29.FRSC & 6  		& 92 & 64&25    & 1297 & 1278 & 19(1.46)  \\ \cline{2-9}%AIS
&30.FX &7.5      & 475 & 423&44   & 4971 & 4775 & 196(3.94)  \\ \hline
\end{tabular}
\end{table}

